LCDnet: A Lightweight Crowd Density Estimation Model for Real-time Video Surveillance

Automatic crowd counting using density estimation has gained significant attention in computer vision research. As a result, a large number of crowd counting and density estimation models using convolution neural networks (CNN) have been published in the last few years. These models have achieved good accuracy over benchmark datasets. However, attempts to improve the accuracy often lead to higher complexity in these models. In real-time video surveillance applications using drones with limited computing resources, deep models incur intolerable higher inference delay. In this paper, we propose (i) a Lightweight Crowd Density estimation model (LCDnet) for real-time video surveillance, and (ii) an improved training method using curriculum learning (CL). LCDnet is trained using CL and evaluated over two benchmark datasets i.e., DroneRGBT and CARPK. Results are compared with existing crowd models. Our evaluation shows that the LCDnet achieves a reasonably good accuracy while significantly reducing the inference time and memory requirement and thus can be deployed over edge devices with very limited computing resources.

==> figures/CRAPK_compare.tex <==


\begin{figure*}
\centering

\includegraphics[width=3.2cm]{figures/JPG/IMG_2.jpg}
\includegraphics[width=3.2cm]{figures/JPG/GT_2.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_MCNN_2.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_CSRNet_2.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_LCDnet_2.jpg}
\\
\includegraphics[width=3.2cm]{figures/JPG/IMG_134.jpg}
\includegraphics[width=3.2cm]{figures/JPG/GT_134.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_MCNN_134.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_CSRNet_134.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_LCDnet_134.jpg}
\\
\includegraphics[width=3.2cm]{figures/JPG/IMG_200.jpg}
\includegraphics[width=3.2cm]{figures/JPG/GT_200.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_MCNN_200.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_CSRNet_200.jpg}
\includegraphics[width=3.2cm]{figures/JPG/Pred_LCDnet_200.jpg}





\caption{Comparison of predictions on on DroneRGBT dataset. The first two columns shows crowd images and their corresponding ground truth. Columns 3-5 shows predictions using MCNN \cite{MCNN_CVPR2016}, CSRNet \cite{CSRNet_CVPR2018}, and LCDnet (ours), respectively.}
\label{fig:CRAPK_compare}
\end{figure*}

==> tables/tab_results_accuracy.tex <==




\begin{table*}[!h]
\centering
\caption{Density Class detection using LCDnet.}
\label{tab:results_accuracy}
\begin{tabular}{p{2cm} p{2cm} p{2cm}  p{1cm} p{2cm} p{2cm} p{2cm} } \toprule
Crowd Density  &\multicolumn{2}{c}{DroneRGBT}  & &\multicolumn{2}{c}{CARPK}  \\ \cmidrule{2-3} \cmidrule{5-6}
        &Count range   &Accuracy (\%)  & &Count range &Accuracy \\ \midrule
Very Low     &0-20     &58.4            &  &0-20     &71.3 \\
Low          &21-50    &78.2            &  &21-50    &82.1 \\
Medium       &51-100   &83.9            &  &51-100   &79.5 \\
High         &101-403  &62.4            &  &101-200  &98.6 \\
\bottomrule
\end{tabular}
\end{table*}
